Reify Your Collection Queries for Modularity and Speed!

Modularity and efficiency are often contradicting requirements, such that programers have to trade one for the other. We analyze this dilemma in the context of programs operating on collections. Performance-critical code using collections need often to be hand-optimized, leading to non-modular, brittle, and redundant code. In principle, this dilemma could be avoided by automatic collection-specific optimizations, such as fusion of collection traversals, usage of indexing, or reordering of filters. Unfortunately, it is not obvious how to encode such optimizations in terms of ordinary collection APIs, because the program operating on the collections is not reified and hence cannot be analyzed. We propose SQuOpt, the Scala Query Optimizer--a deep embedding of the Scala collections API that allows such analyses and optimizations to be defined and executed within Scala, without relying on external tools or compiler extensions. SQuOpt provides the same "look and feel" (syntax and static typing guarantees) as the standard collections API. We evaluate SQuOpt by re-implementing several code analyses of the Findbugs tool using SQuOpt, show average speedups of 12x with a maximum of 12800x and hence demonstrate that SQuOpt can reconcile modularity and efficiency in real-world applications.

==> graphs/EvalSummaryTable.tex <==
\begin{tabular}{l*{7}{r}}\toprule
&M ($1/2$) &S (1/$3^-$)&H ($2/3^o$)&H' ($2/3^x$)&O ($1/3^o$)&X ($3^o/3^x$)&T ($1/3^x$)\\\midrule
\tablerowsize Geometric means of performance ratios
\input{\graphPath{speedups}}
\addlinespace
\bottomrule
\end{tabular}


==> graphs/EvalTable.tex <==
\begin{tabular}{rlrrrrrrrrrrr}\toprule
&&\multicolumn{5}{c}{Performance (ms)}&\multicolumn{3}{c}{Performance ratios} \\\cmidrule(lr){3-7}\cmidrule(lr){8-10}
%
Id&Description&1&2& $3^-$&$3^o$&$3^x$&M ($1/2$) &H ($2/3^o$)&T ($1/3^x$)\\\midrule

%
%
\input{\graphPath{newTable}}
\addlinespace
%
%
\bottomrule
\end{tabular}
\\
\captionEvalTable


==> graphs/evalRes.tex <==

\newcommand{\avgRealTimeFb}{43.52}
\newcommand{\avgRealSdFb}{1.38}
\newcommand{\avgUserTimeFb}{90.74}
\newcommand{\avgUserSdFb}{1.26}
\newcommand{\avgRealTimeLos}{17.16}
\newcommand{\avgRealSdLos}{0.25}
\newcommand{\avgUserTimeLos}{31.27}
\newcommand{\avgUserSdLos}{0.69}
\newcommand{\avgRealTimeLosOpt}{22.57}
\newcommand{\avgRealSdLosOpt}{1.05}
\newcommand{\avgUserTimeLosOpt}{40.89}
\newcommand{\avgUserSdLosOpt}{1.18}


==> graphs/evalResLos.tex <==

\newcommand{\kZrememberedSampleLoops}{10}
\newcommand{\qZmaxLoops}{50}
\newcommand{\thetaZmaxCov}{0.1}
\newcommand{\readingClassFilesTime}{4755.32 \pm 141.66}
\newcommand{\queryCOVARIANTCOMPARETO}{$1$}
\newcommand{\speedupTCOVARIANTCOMPARETO}{4.4x}
\newcommand{\queryGCCALL}{$2$}
\newcommand{\speedupTGCCALL}{9.5x}
\newcommand{\queryPROTECTEDFIELD}{$3$}
\newcommand{\speedupTPROTECTEDFIELD}{9.8x}
\newcommand{\queryRUNFINALIZERSONEXIT}{$4$}
\newcommand{\speedupTRUNFINALIZERSONEXIT}{51x}
\newcommand{\queryNOTCLONEABLE}{$5$}
\newcommand{\speedupTNOTCLONEABLE}{61x}
\newcommand{\queryCOVARIANTEQUALS}{$6$}
\newcommand{\speedupTCOVARIANTEQUALS}{147x}
\newcommand{\queryFINALIZERNOTPROTECTED}{$7$}
\newcommand{\speedupTFINALIZERNOTPROTECTED}{1070x}
\newcommand{\queryDONTCATCHIMSE}{$8$}
\newcommand{\speedupTDONTCATCHIMSE}{12800x}
\newcommand{\queryURUNINITREADCALLEDFROMSUPERCONSTRUCTOR}{$9^R$}
\newcommand{\speedupTURUNINITREADCALLEDFROMSUPERCONSTRUCTOR}{0.9x}
\newcommand{\queryMSPKGPROTECT}{$10^R$}
\newcommand{\speedupTMSPKGPROTECT}{1.0x}
\newcommand{\querySICINNERSHOULDBESTATICANON}{$11^R$}
\newcommand{\speedupTSICINNERSHOULDBESTATICANON}{1.0x}
\newcommand{\queryITAINEFFICIENTTOARRAY}{$12^R$}
\newcommand{\speedupTITAINEFFICIENTTOARRAY}{1.1x}
\newcommand{\queryBXBOXINGIMMEDIATELYUNBOXEDTOPERFORMCOERCION}{$13^R$}
\newcommand{\speedupTBXBOXINGIMMEDIATELYUNBOXEDTOPERFORMCOERCION}{1.2x}
\newcommand{\queryDMILONGBITSTODOUBLEINVOKEDONINT}{$14^R$}
\newcommand{\speedupTDMILONGBITSTODOUBLEINVOKEDONINT}{1.3x}
\newcommand{\queryDPDOINSIDEDOPRIVILEGED}{$15^R$}
\newcommand{\speedupTDPDOINSIDEDOPRIVILEGED}{1.5x}
\newcommand{\queryMSSHOULDBEFINAL}{$16^R$}
\newcommand{\speedupTMSSHOULDBEFINAL}{1.8x}
\newcommand{\querySEBADFIELDINNERCLASS}{$17^R$}
\newcommand{\speedupTSEBADFIELDINNERCLASS}{6.9x}
\newcommand{\querySWSWINGMETHODSINVOKEDINSWINGTHREAD}{$18^R$}
\newcommand{\speedupTSWSWINGMETHODSINVOKEDINSWINGTHREAD}{13x}
\newcommand{\queryFIUSELESS}{$19^R$}
\newcommand{\speedupTFIUSELESS}{541x}
\newcommand{\MaxDevExp}{28.7}
\newcommand{\MaxStdErrExp}{9.1}
\newcommand{\minInvInterpOver}{0.3}
\newcommand{\geoMeanInterpOver}{1.2}
\newcommand{\maxInvInterpOver}{12.9}
\newcommand{\minInterpOver}{0.1}
\newcommand{\maxInterpOver}{3.4}
\newcommand{\minOptimTime}{3.5}
\newcommand{\avgOptimTime}{54.8}
\newcommand{\stdDevOptimTime}{85.5}
\newcommand{\maxOptimTime}{381.7}
\newcommand{\minOptimSpeedup}{1.2x}
\newcommand{\maxOptimSpeedup}{12800x}
\newcommand{\nSpeededUpQueries}{15}
\newcommand{\speedupBigThreshold}{5}
\newcommand{\nBigSpeededUpQueries}{10}
\newcommand{\randomQueryCount}{11}
\newcommand{\manualQueryCount}{8}
\newcommand{\queryCount}{19}
\newcommand{\avgSpeedupT}{12x}
\newcommand{\maxSpeedupT}{12800x}


==> graphs/indexes.tex <==

Method name&$97.99$&$\pm$&$2.94$\\
Exception handlers&$179.29$&$\pm$&$3.21$\\
Instruction type&$4166.49$&$\pm$&$202.85$\\


==> graphs/newTable.tex <==

$1$&{\tablerowsize Covariant compareTo() defined}&1.1&1.3&0.85&0.26&0.26&0.9&5.0&4.4\\
$2$&{\tablerowsize Explicit garbage collection call}&496&258&1176&1150&52&1.9&0.2&9.5\\
$3$&{\tablerowsize Protected field in final class}&11&1.1&11&1.2&1.2&10.0&1.0&9.8\\
$4$&{\tablerowsize Explicit runFinalizersOnExit() call}&509&262&1150&1123&10.0&1.9&0.2&51\hphantom{.0}\\
$5$&{\tablerowsize clone() defined in non-Cloneable class}&29&14&55&46&0.47&2.1&0.3&61\hphantom{.0}\\
$6$&{\tablerowsize Covariant equals() defined}&29&15&23&9.7&0.20&1.9&1.6&147\hphantom{.0}\\
$7$&{\tablerowsize Public finalizer defined}&29&12&28&8.0&0.03&2.3&1.5&1070\hphantom{.0}\\
$8$&{\tablerowsize Dubious catching of IllegalMonitorStateException}&82&72&110&28&0.01&1.1&2.6&12800\hphantom{.0}\\
$9^R$&{\tablerowsize Uninit. field read during construction of super}&896&367&3017&960&960&2.4&0.4&0.9\\
$10^R$&{\tablerowsize Mutable static field declared public}&9527&9511&9115&9350&9350&1.0&1.0&1.0\\
$11^R$&{\tablerowsize Refactor anon. inner class to static}&8804&8767&8718&8700&8700&1.0&1.0&1.0\\
$12^R$&{\tablerowsize Inefficient use of toArray(Object[])}&3714&1905&4046&3414&3414&2.0&0.6&1.1\\
$13^R$&{\tablerowsize Primitive boxed and unboxed for coercion}&3905&1672&5044&3224&3224&2.3&0.5&1.2\\
$14^R$&{\tablerowsize Double precision conversion from 32 bit}&3887&1796&5289&3010&3010&2.2&0.6&1.3\\
$15^R$&{\tablerowsize Privileged method used outside doPrivileged}&505&302&1319&337&337&1.7&0.9&1.5\\
$16^R$&{\tablerowsize Mutable public static field should be final}&13&6.2&12&7.0&7.0&2.0&0.9&1.8\\
$17^R$&{\tablerowsize Serializable class is member of non-ser. class}&12&0.77&0.94&1.8&1.8&16\hphantom{.0}&0.4&6.9\\
$18^R$&{\tablerowsize Swing methods used outside Swing thread}&577&53&1163&45&45&11\hphantom{.0}&1.2&13\hphantom{.0}\\
$19^R$&{\tablerowsize Finalizer only calls super class finalize}&55&13&73&11&0.10&4.4&1.1&541\hphantom{.0}\\


==> graphs/queryTables.tex <==


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{table}
\begin{tabular}{p{7cm}r}\toprule
Abstraction & Used \\ \midrule
%
All fields in all class files	& 4\\
All methods in all class files	& 3\\
All method bodies in all class files	& 3\\
All instructions in all method bodies and their bytecode index	& 5\\
Sliding window (size $n$) over all instructions (and their index) &	3\\
\bottomrule
\end{tabular}\\
\nocaptionrule\caption{Description of abstractions removed during hand-optimization and number of queries where the abstraction is used (and optimized away).}
\label{table:implemented-abstractions}
\end{table}

\newcommand{\captionEvalTable}{
Implementations and speedups are as defined in Sec.~\ref{sec:implemenationsandspeedups}.
Queries marked with $^R$ were selected by random sampling.
\pg{Extend caption. Reconsider which columns to show. H is important to
acknowledge our limitations (if we want). Resort queries.}
}
\newcommand{\tablerowsize}{\scriptsize}
\begin{table*}[tb]
\begin{center}
\input{\graphPath{EvalTable}}
\end{center}
\nocaptionrule\caption{Performance results.}
\label{table:performance}
\end{table*}

\begin{table*}[tb]
\begin{center}
\input{\graphPath{EvalSummaryTable}}
\\
\pg{Description}
\end{center}
\nocaptionrule\caption{Average performance ratios.}
\label{table:performanceAvg}
\end{table*}

\begin{extraEval}
\begin{table*}[tb]
\begin{center}
\begin{tabular}{l*{3}{r@{}c@{}l}r*{2}{r@{}c@{}l}}\toprule
Name&\multicolumn{3}{c}{Base impl.\ (in ms)}&\multicolumn{3}{c}{Modular impl}&\multicolumn{3}{c}{Optimiz.\ time}&IS&\multicolumn{3}{c}{OS}&\multicolumn{3}{c}{OS-Opt}\\\midrule
\input{\graphPath{table}}
\bottomrule
\end{tabular}
\end{center}
\nocaptionrule\caption{Old performance results table}
\label{table:performanceOld}
\end{table*}
\end{extraEval}


==> graphs/speedups.tex <==

{}&2.4x&1.2x&0.8x&5.1x&1.9x&6.3x&12x\\


==> macros.tex <==
\usepackage{ifxetex}

\usepackage{eurosym}
\ifxetex
\else
\usepackage[utf8]{inputenc}
\DeclareUnicodeCharacter{20AC}{\euro}
\usepackage[T1]{fontenc}
\usepackage{amssymb}
\fi
\usepackage{fixltx2e}[2005/12/01]
\usepackage[unicode=true]{hyperref}
\usepackage[scaled=0.88]{beramono} %
\usepackage{amsmath}
\usepackage{bookmark}
\usepackage{tikz}
\usepackage{stmaryrd}
\usepackage{booktabs}
\newcommand{\smartParagraph}[1]{\textbf{#1}}

\usepackage{listings}
%
%
%
\lstdefinelanguage{scala}{
  morekeywords={%
	  abstract,case,catch,class,def,do,else,extends,%
	  false,final,finally,for,forSome,if,implicit,import,lazy,%
	  match,new,null,object,override,package,private,protected,%
	  return,sealed,super,this,throw,trait,true,try,type,%
	  val,var,while,with,yield},
  otherkeywords={=>,<-,<\%,<:,>:,\#,@},
  sensitive=true,
  morecomment=[l]{//},
  morecomment=[n]{/*}{*/},
  morestring=[b]",
  morestring=[b]',
  morestring=[b]"""
}[keywords,comments,strings]

%
%
%
%
%
%
%
%
%
%
%
%
%

%
\lstset{
    language=Scala,%
%
%
%
%
%
%
%
    tabsize=2,%
    %
    %
    commentstyle=\itshape,%
    keywordstyle=\bfseries,%
    mathescape=true,%
    escapechar=£,%
    %
%
%
    firstnumber=0,%
%
    numberstyle=\tiny,%
}
\lstset{%
basicstyle=\scriptsize\ttfamily,	%
%
%
%
%
%
%
identifierstyle=,%
%
stringstyle=\ttfamily, %
showstringspaces=false, %
language=Scala,
%
breakindent=2ex,   %
breaklines,
breakatwhitespace,
breakautoindent=true,
keepspaces
%
}



%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\newcommand{\code}[1]{%
    \lstinline[basicstyle=\footnotesize\ttfamily]^#1^}
%

\newcommand{\mynote}[2]
    {\textcolor{red}{
     {\bfseries\sffamily\scriptsize#1}
     {\small$\blacktriangleright$\textsf{\emph{#2}}$\blacktriangleleft$}}}
\renewcommand{\mynote}[2]{}

\newcommand{\TODO}{\mynote}
\newcommand{\pg}{\TODO{PG}}
\newcommand{\tr}{\TODO{TR}}
\newcommand{\ko}{\TODO{KO}}
\newcommand{\chk}{\TODO{CK}}
\newcommand{\mei}{\TODO{ME}}
\newcommand{\rmi}{\TODO{RM}}

\providecommand{\nocaptionrule}{} %
%
\newcommand{\ExpWrap}{\mathit{Lift}}
%
%
\newcommand{\LoS}{\textsc{SQuOpt}} %
\newcommand{\LoSDef}{\LoS, the Scala QUery OPTimizer}
%
%
\newcommand{\LINQ}{\textsc{Linq}}

%
%
\lstset{literate={{<-}{{$\gets$}}1 {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 { => }{{$\Rightarrow$}}1 { -> }{{$\rightarrow$}}1 {...}{{\ldots} }2}}
\newcommand{\codem}[1]{\mbox{\code{#1}}}
\hypersetup{breaklinks=true, pdfborder={0 0 0}}

%
%
%
%
%

\newcommand{\intersect}{\wedge}
\providecommand{\IEEEPARstart}[2]{#1#2}


==> pepm13/caseStudyDiscussion.tex <==
In this section we discuss the degree to which \LoS\ fulfilled our original design goals, and the conclusions
for host and domain-specific language design.

\subsection{What worked well}
Several features of Scala contributed greatly to the success we achieved. With implicit conversions, the lifting can be made mostly transparent. The advanced type system features were quite helpful to make the expression tree representation typed. The fact that for-comprehensions are desugared \emph{before} type inference and type checking was also a prerequisite for automatic lifting. The syntactic expressiveness and uniformity of Scala, in particular the fact that custom types can have the same look-and-feel as primitive types, were also vital to lift expressions on primitive types.

%
\subsection{Limitations}
\label{sec:limitations}
Despite these positive experiences and our experimental success, our embedding has a few significant limitations.

The first limitation is that we only lift a subset of Scala, and some interesting features are missing.
We do not support \emph{statements} in nested blocks in our queries, but this could be implemented reusing techniques from Delite~\citep{Rompf11BBlocks}.
%
More importantly for queries, \emph{pattern matching} cannot be supported by deep embedding similar to ours. In contrast to for-comprehension syntax, pattern matching is desugared only \emph{after} type checking \cite{Emir07Patterns}, which prevents us from lifting pattern matching notation. More specifically, because an extractor \cite{Emir07Patterns} cannot return the representation of a result value (say \code{Exp[Boolean]}) to later evaluate; it must produce its final result at pattern matching time. There is initial work on ``virtualized pattern matching''\footnote{\url{http://stackoverflow.com/questions/8533826/what-is-scalas-experimental-virtual-pattern-matcher}}, and we hope to use this feature in future work.

We also experienced problems with operators that cannot be overloaded, such as \code{==} or \code{if-else} and with lifting methods in \code{scala.Any}, which forced us to provide alternative syntax for these features in queries. The  Scala-virtualized project \citep{Moors12Virtualized} aims to address these limitations; unfortunately, it advertises no change on the other problems we found, which we subsequently detail.

%

It would also be desirable if we could enforce the absence of side effects in queries, but since Scala, like most practical programming languages except Haskell, does not track side effects in the type system this does not seem to be possible. 
%

Finally, compared to \emph{lightweight modular staging}~\citep{rompf2010lightweight} (the foundation of Delite) and to polymorphic embedding~\citep{hofer08polymorphic}, we have less static checking for some programming errors when writing queries; the recommended way to use Delite is to write a DSEL program in one trait, in terms of the DSEL interface only, and combine it with the implementation in another trait. In polymorphic embedding, the DSEL program is a function of the specific implementation (in this case, semantics).
Either approach ensures that the DSL program is \emph{parametric} in the implementation, and hence cannot refer to details of a specific implementation.
However, we judged the syntactic overhead for the programmer to be too high to use those techniques -- in our implementation we rely on encapsulation and on dynamic checks at query construction time to achieve similar guarantees.

The choice of interpreting expressions turned out to be a significant performance limitation. It could likely be addressed by using Delite and lightweight modular staging instead, but we wanted to experiment with how far we can get \emph{within} the language in a well-typed setting.

%
%

\subsection{What did not work so well: Scala type inference}
\label{sec:ScalaLessons}

%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%


%
%


%

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%

%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
When implementing our library, we often struggled against limitations and bugs in the Scala compiler, especially regarding type inference and its interaction with implicit resolution, and we were often constrained by its limitations. Not only Scala's type inference is not complete, but we learned that its behavior is only specified by the behavior of the current implementation: in many cases where there is a clear desirable solution, type inference fails or finds an incorrect substitution which leads to a type error. Hence we cannot distinguish, in the discussion, the Scala language from its implementation.
We regard many of Scala's type inference problems as bugs, and reported them as such when no previous bug report existed, as noted in the rest of this section. Some of them are long-standing issues, others of them were accepted, for other ones we received no feedback yet at the time of this writing, and another one was already closed as WONTFIX, indicating that a fix would be possible but have excessive complexity for the time being.\footnote{\url{https://issues.scala-lang.org/browse/SI-2551}}.

\smartParagraph{Overloading}
The code in Fig.~\ref{fig:reifiedQuery} uses the lifted \code{BookData} constructor. Two definitions of \code{BookData} are available, with signatures \code{BookData(String, String, Int)} and \code{BookData(Exp[String], Exp[String], Exp[Int])}, and it seems like the Scala compiler should be able to choose which one to apply using overload resolution. This however is not supported simply because the two functions are defined in different scopes\footnote{\url{https://issues.scala-lang.org/browse/SI-2551}}, hence importing \code{BookData(Exp[String], Exp[String], Exp[Int])} shadows locally the original definition.
%
%
%
%
%

%
%

%
%

\smartParagraph{Type inference vs implicit resolution}
The interaction between type inference and implicit resolution is a hard problem, and Scalac has also many bugs, but the current situation requires further research; for instance, there is not even a specification for the behavior of type inference\footnote{\url{https://issues.scala-lang.org/browse/SI-5298?focusedCommentId=55971##comment-55971}, reported by us.}.

As a consequence, to the best of our knowledge some properties of type inference have not been formally established.
For instance, a reasonable user expectation is that removing a call to an implicit conversion does not alter the program, if it is the only implicit conversion with the correct type in scope, or if it is more specific than the others~\citep[Ch. 21]{Odersky11book}. This is not always correct, because removing the implicit conversion reduces the information available for the type inference algorithm; we observed multiple cases\footnote{\url{https://issues.scala-lang.org/browse/SI-5592}, reported by us.} where type inference becomes unable to figure out enough information about the type to trigger implicit conversion.

We also consider significant that Scala 2.8 required making both type inference and implicit resolution more powerful, specifically in order to support the collection library~\citep[Sec 21.7]{Moors10TCP,Odersky11book}; further extensions would be possible and desirable.
For instance, if type inference were extended with higher-order unification\footnote{\url{https://issues.scala-lang.org/browse/SI-2712}}~\citep{Pfenning88}, it would better support a part of our DSL interface (not discussed in this paper) by removing the need for type annotations.
%

%
%

%
%

\smartParagraph{Nested pattern matches for GADTs in Scala}
Writing a typed decomposition for \code{Exp} requires pattern-matching support for generalized algebraic datatypes (GADTs). We found that support for GADTs in Scala is currently insufficient. \citet{Emir07Patterns} define the concept of \emph{typecasing}, essentially a form of pattern-matching limited to non-nested patterns, and demonstrate that Scala supports typecasing on GADTs in Scala by demonstrating a typed evaluator; however, typecasing is rather verbose for deep patterns, since one has to nest multiple pattern-matching expressions.
When using normal pattern matches, instead, the support for GADT seems much weaker.\footnote{Due to bug \url{https://issues.scala-lang.org/browse/SI-5298?focusedCommentId=56840##comment-56840}, reported by us.}
%
Hence one has to choose between support for GADT and the convenience of nested pattern matching.
A third alternative is to ignore or disable compiler warnings, but we did not consider this option. \pg{I would add that: ``Apparently this was instead the option chosen for Scala-virtualized~\citep{Moors12Virtualized}'', but I'd like to ask Adriaan first.}

%

%

%
%
%

%
%

\smartParagraph{Implicit conversions do not chain}
While implicit conversions by default do not chain, it is sometimes convenient to allow chaining selectively.
For instance, let us assume a context such that \code{a: Exp[A]}, \code{b: Exp[B]} and \code{c: Exp[C]}.
In this context, let us consider again how we lift tuples. We have seen that the expression \code{(a, b)} has type \code{(Exp[A], Exp[B])} but can be converted to \code{Exp[(A, B)]} through an implicit conversion. Let us now consider \emph{nested} tuples, like \code{((a, b), c)}: it has type \code{((Exp[A], Exp[B]), Exp[C])}, hence the previous conversion cannot be applied to this expression.

\citet[Ch.~21]{Odersky11book} describe a pattern which can address this goal. Using this pattern, to lift pairs, we must write an implicit conversion from pairs of elements which can be \emph{implicitly converted} to expressions. Instead of requiring
\code{(Exp[A], Exp[B])}, the implicit conversion should require \code{(A, B)} with the condition that \code{A} can be converted to \code{Exp[A']} and \code{B} to \code{Exp[B']}. This conversion solves the problem if applied explicitly,
but the compiler refuses to apply it implicitly, again because of type inference issues\footnote{\url{https://issues.scala-lang.org/browse/SI-5651}, reported by us.}.

Because of this type inference limitations, we failed to provide support for reifying code like \code{((a, b), c)}\footnote{One could of course write a specific implicit conversions for \emph{this} case; however, \code{(a, (b, c))} requires already a different implicit conversion, and there are infinite ways to nest pairs, let alone tuples of bounded arity.}.
%

%
%
%

%
%

%
%
%
%
%
%
%


\smartParagraph{Error messages for implicit conversions}
The enrich-my-library pattern has the declared goal to allow to extend existing libraries \emph{transparently}. However, implementation details shine however through when a user program using this feature contains a type error. When invoking a method would require an implicit conversion which is not applicable, the compiler often just reports that the method is not available. The recommended approach to debugging such errors is to manually add the missing implicit conversion and investigating the type error~\citep[Ch.~21.8]{Odersky11book}, but this destroys the transparency of the approach when creating or modifying code.
\pg{Is our suggestion helpful? Is our complaint helpful without the suggestion?} We believe this could be solved in principle by research on error reporting: the compiler could automatically insert all implicit conversions enabling the method calls and report corresponding errors, even if at some performance cost.
%


%

\subsection{Lessons for language embedders}
Various domains, such as the one considered in our case study, allow powerful domain-specific optimizations. Such optimizations often are hard to express in a compositional way, hence they cannot be performed while building the query but must be expressed as global optimizations passes.
For those domains, deep embedding is key to allow significant optimizations.
%
On the other hand, deep embedding requires to implement an interpreter or a compiler.

On the one hand, interpretation overhead is significant in Scala, even when
using HOAS to take advantage of the metalevel implementation of argument access.
%
%

Instead of interpreting a program, one can compile a DSEL program to Scala and load it, as done by \citet{Rompf11BBlocks};
while we are using this approach, the disadvantage is the compilation delay,
especially for Scala whose compilation process is complex and time-consuming.
Possible alternatives include generating bytecode directly or combining
interpretation and compilations similarly to tiered JIT compilers, where only
code which is executed often is compiled. We plan to investigate such
alternatives in future work.
%

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%

%


==> pepm13/caseStudyGoals.tex <==
While the basic idea of deep embedding is well known, it is not obvious how to realize deep embedding
when considering the following additional goals:

\begin{itemize}
\item To support users adopting \LoS, a generic \LoS\ query should share the ``look and feel'' of the ordinary collections API: In particular, query syntax should remain mostly unchanged. In our case, we want to preserve  Scala's \emph{for-comprehension}\footnote{Also known as \emph{for expressions}~\citep[Ch.~23]{Odersky11book}.} syntax and its notation
 for anonymous functions.
 %
 %
 %
 \item Again to support users adopting \LoS, a generic \LoS\ query should not only share the syntax of the ordinary collections API; it should also be well-typed if and only if the corresponding ordinary query is well-typed.
 This is particularly challenging in the Scala collections
 library due to its deep integration with advanced type-system features, such as higher-kinded generics
 and implicit objects~\citep{odersky2009fighting}. For instance, calling \code{map} on a \code{List} will return a \code{List}, and calling \code{map} on a \code{Set}
 will return a \code{Set}. Hence the object-language representation and the
 transformations thereof should be as ``typed'' as possible. This precludes, among others, a first-order
 representation of object-language variables as strings.
 \item \LoS\ should be interoperable with ordinary Scala code and Scala collections. For instance, it should
 be possible to call normal non-reified functions within a \LoS\ query, or mix native Scala queries and \LoS\ queries.
%
%
 \item The performance of \LoS\ queries should be reasonable even without optimizations. A non-optimized \LoS\ query
 should not be dramatically slower than a native Scala query. Furthermore, it should be possible to create new queries at run time and execute them without excessive overhead.
 This goal limits the options of applicable interpretation or compilation techniques.
\end{itemize}
\chk{these goals are not really justified, but that may be too late to change}
 
We think that these challenges characterize deep embedding of queries on collections as a \emph{critical} case study~\citep{flyvbjerg06five} for DSL embedding.
That is, it is so challenging that embedding techniques successfully used in this case are likely to be successful on a broad range of other DSLs.
From the case study, we report the successes and failures of achieving these goals in \LoS. 


==> pepm13/caseStudyImpl.tex <==
%
%
%
%
To optimize a query as described in the previous section, {\LoS} needs to reify, optimize and execute queries. 
Our implementation assigns responsibility for these steps to three main components: A generic library for reification and execution of general Scala expressions, a more specialized library for reification and execution of query operators, and a dedicated query optimizer.
Queries need then to be executed through either compilation (already discussed in
Sec.~\ref{sec:execution}) or interpretation (to discuss in Sec.~\ref{sec:interpretation}).
We describe the implementation in more detail in the rest of this section. The full implementation is also available online\footnote{\url{http://www.informatik.uni-marburg.de/~pgiarrusso/SQuOpt}}.
%

A core idea of {\LoS} is to reify Scala code as a data structure in memory. A programmer could directly create instances of that data structure, but we also provide a more convenient interface based on advanced Scala features such as implicit conversions and type inference. That interface allows to automatically reify code with a minimum of programmer annotations, as shown in the examples in Sec.~\ref{sec:solution}. Since this is a case study on Scala's support for deep embedding of DSLs, we also describe in this section how Scala supports our task. In particular, we report on techniques we used and issues we faced.

%
\subsection{Representing expression trees}
\label{subsec:repexptrees}
In the previous section, we have seen that expressions that would have type \code{T} in a native Scala query are reified and have type \code{Exp[T]} in \LoS. The generic type \code{Exp[T]} is the base for our reification of Scala expression as expression trees, that is, as data structures in memory. We provide a subclass of \code{Exp[T]} for every different form of expression we want to reify. For example, in Fig.~\ref{fig:query} the expression \code{author.firstName + " " + author.lastName} must be reified even though it is not collection-related, for otherwise the optimizer could not see whether \code{author} is used. Knowing this is needed for instance to remove variables which are bound but not used. Hence, this expression is reified as \code{StringConcat(StringConcat(AuthorFirstName(author), Const(" ")), AuthorLastName(author))}. This example uses the constructors of the following subclasses of \code{Exp[T]} to create the expression tree.

\begin{lstlisting}
case class Const[T](t: T) extends Exp[T]

case class StringConcat(str1: Exp[String],
                        str2: Exp[String])
  extends Exp[String]

case class AuthorFirstName(t: Exp[Author])
  extends Exp[String]

case class AuthorLastName(t: Exp[Author])
  extends Exp[String]
\end{lstlisting}

Expression nodes additionally implement support code for tree traversals to support optimizations, which we omit here.

This representation of expression trees is well-suited for a representation of the structure of expressions in memory and also for pattern matching (which is automatically supported for case classes in Scala), but inconvenient for query writers. In fact, in Fig.~\ref{fig:titlefiltersquopt} and \ref{fig:reifiedQuery}, we have seen that {\LoS} provides a much more convenient front-end: The programmer writes almost the usual code for type \code{T} and {\LoS} converts it automatically to \code{Exp[T]}.

\subsection{Lifting first-order expressions}

We call the process of converting from \code{T} to \code{Exp[T]} \emph{lifting}. Here we describe how we lift first-order expressions -- Scala expressions that do
not contain anonymous function definitions.

To this end, consider again the fragment \code{author.firstName + " " + author.lastName}, now in the context of the {\LoS}-enabled query in Fig.~\ref{fig:reifiedQuery}. It looks like a normal Scala expression, even syntactically unchanged from Fig.~\ref{fig:query}. However, evaluating that code in the context of Fig.~\ref{fig:reifiedQuery} does not concatenate any strings, but creates an expression tree instead. Although the code looks like the same expression, it has a different \emph{type}, \code{Exp[String]} instead of \code{String}. This difference in the type is caused by the context: The variable \code{author} is now bound in a {\LoS}-enabled query and therefore has type \code{Exp[Author]} instead of \code{Author}. We can still access the \code{firstName} field of \code{author}, because expression trees of type \code{Exp[T]} provide the same interface as values of type \code{T}, except that all operations return expressions trees instead of values.

To understand how an expression tree of type \code{Exp[T]} can have the same interface as a value of type \code{T}, we consider two expression trees \code{str1} and \code{str2} of type \code{Exp[String]}. The implementation of lifting differs depending on the kind of expression we want to lift.

\smartParagraph{Method calls and operators}
In our example, the operator \code{+} should be available on \code{Exp[String]}, but not on \code{Exp[Boolean]}, because \code{+} is available on \code{String} but not on \code{Boolean}.
Furthermore, we want \code{str1 + str2} to have type \code{Exp[String]} and to evaluate not to a string concatenation but to a call of \code{StringConcat}, that is, to an expression tree which \emph{represents} \code{str1 + str2}. This is a somewhat unusual requirement, because usually, the interface of a generic type does not depend on the type parameters.

To provide such operators and to encode expression trees, we use \emph{implicit conversions} in a similar style as \citet{rompf2010lightweight}. Scala allows to make expressions of a type \code{T} implicitly convertible to a different type \code{U}. To this end, one must declare an \emph{implicit conversion function} having type \code{T => U}. Calls to such functions will be inserted by the compiler when required to fix a type mismatch between an expression of type \code{T} and a context expecting a value of type \code{U}. In addition, a method call \code{e.m(args)} can trigger the conversion of \code{e} to a type where the method \code{m} is present\footnote{For the exact rules, see \citet[Ch.~21]{Odersky11book} and \citet{ScalaRef}.}. Similarly, an operator usage, as in \code{str1 + str2}, can also trigger an implicit conversion: an expression using an operator, like \code{str1 + str2}, is desugared to the method call \code{str1.+(str2)}, which can trigger an implicit conversion from \code{str1} to a type providing the \code{+} method. Therefore from now on we do not distinguish between operators and methods.

To provide the method \code{+} on \code{Exp[String]}, we define an implicit conversion from \code{Exp[String]} to a new type providing a \code{+} method which creates the appropriate expression node.
\begin{lstlisting}
implicit def expToStringOps(t: Exp[String]) =
  new StringOps(t)
class StringOps(t: Exp[String]) {
  def +(that: Exp[String]): Exp[String] =
    StringConcat(t, that)
}
\end{lstlisting}
This is an example of the well-known Scala \emph{enrich-my-library pattern}\footnote{Also known as \emph{pimp-my-library} pattern.}~\citep{OderskyPimpLib}.
 
With these declarations in scope, the Scala compiler rewrites \code{str1 + str2} to
\code{expToStringOps(str1).+(str2)}, which evaluates to \code{StringConcat(str1, str2)} as desired.
Note that the implicit conversion function \code{expToStringOps} is not applicable to \code{Exp[Boolean]} because it explicitly specifies the receiver of the \code{+}-call to have type \code{Exp[String]}.
In other words, expressions like \code{str1 + str2} are now \emph{lifted} on the level of expression trees in a type-safe way. For brevity, we refer to the defined operator as \code{Exp[String].+}.

\smartParagraph{Literal values}
However, a string concatenation might also include constants, as in \code{str1 + "foo"} or \code{"bar" + str1}.
To lift \code{str1 + "foo"}, we introduce a lifting for constants which wraps them in a \code{Const} node:

\begin{lstlisting}
implicit def pure[T](t: T): Exp[T] = Const(t)
\end{lstlisting}
%

The compiler will now rewrite \code{str1 + "foo"} to \code{expToStringOps(str1) + pure("foo")}.
%
%
Similarly, \code{author. firstName + " " + author.lastName} is rewritten to \code{(expToStringOps(author.firstName) + pure(" ")) + author.lastName}.
Note how the implicit conversions cooperate successfully to lift the expression.

Analogously, it would be convenient if the similar expression \code{"bar" + str1} would be rewritten to \code{expToStringOps(pure("bar")) + str1}, but this is not the case, because implicit coercions are not chained automatically in Scala.
Instead, we have to manually chain existing implicit conversions into a new one:
\begin{lstlisting}
implicit def toStringOps(t: String) = expToStringOps(pure(t)) 
\end{lstlisting}
so that \code{"bar" + str1} is rewritten to \code{toStringOps("bar") + str1}.

\smartParagraph{User-defined methods}
Calls of user-defined methods like \code{author.firstName} are lifted the same way as calls to built-in methods such as string concatenation shown earlier. For the running example, the following definitions are necessary to lift the methods from \code{Author} to \code{Exp[Author]}.

\begin{lstlisting}
package schema.squopt

implicit def expToAuthorOps(t: Exp[Author]) =
  new AuthorOps(t)
implicit def toAuthorOps(t: Author) =
  expToAuthorOps(pure(t))
class AuthorOps(t: Exp[Author]) {
  def firstName: Exp[String] = AuthorFirstName(t)
  def lastName: Exp[String] = AuthorLastName(t)
}
\end{lstlisting}

\code{Author} is not part of {\LoS} or the standard Scala library but an application-specific class, hence it is not possible
to pre-define the necessary lifting code as part of {\LoS}. Instead, the application programmer needs to provide this code to connect {\LoS} to his application. To support the application programmer with this tedious task, we provide a code generator which discovers the interface of a class through reflection on its compiled version and generates the boilerplate code such as the one above for \code{Author}. It also generates 
the application-specific expression tree types such as \code{AuthorFirstName} as shown in Sec.~\ref{subsec:repexptrees}.
In general, query writers need to generate and import the boilerplate lifting code for all application-specific types they want to use in a {\LoS} query.

If desired, we can exclude some methods to \emph{restrict} the language supported in our deeply embedded programs. For instance \LoS{} requires the user to write side-effect-free queries, hence we do not lift methods which perform side effects.

Using similar techniques, we can also lift existing functions and implicit conversions.



\smartParagraph{Tuples and other generic constructors}
The techniques presented above for the lifting of method calls rely on overloading the name of the method with a signature that involves \code{Exp}. Implicit resolution (for method calls) will then choose our lifted version of the function or method to satisfy the typing requirements of the context or arguments of the call. Unfortunately, this technique does not work for tuple constructors, which, in Scala, are not resolved like ordinary calls. Instead, support for tuple types is hard-wired into the language, and tuples are always created by the predefined tuple constructors.

For example, the expression \code{(str1, str2)} will always call Scala's built-in \code{Tuple2} constructor and correspondingly have type \code{(Exp[String], Exp[String])}. We would prefer that it calls a lifting function and produces an expression tree of type \code{Exp[(String, String)]} instead.

Even though we cannot intercept the call to \code{Tuple2}, we can add an implicit conversion to be called \emph{after} the tuple is constructed.

\begin{lstlisting}
implicit def tuple2ToTuple2Exp[A1, A2]
    (tuple: (Exp[A1], Exp[A2])): LiftTuple2[A1, A2] =
  LiftTuple2[A1, A2](tuple._1, tuple._2)
case class LiftTuple2[A1, A2](t1: Exp[A1], t2: Exp[A2]) extends Exp[(A1, A2)]
\end{lstlisting}

We generate such conversions for different arities with a code generator. These conversions will be used only when the context requires an expression tree. Note that this technique is only applicable because tuples are generic and support arbitrary components, including expression trees.

In fact, we use the same technique also for other generic constructors to avoid problems associated with shadowing of constructor functions. For example, an implicit conversion is used to lift \code{Seq[Exp[T]]} to \code{Exp[Seq[T]]}: code like \code{Seq(str1, str2)} first constructs a sequence of expression trees and then wraps the result with an expression node that describes a sequence.
%

\smartParagraph{Subtyping}
So far, we have seen that for each first-order method \code{m} operating on instances of \code{T}, we can create a corresponding method which operates on \code{Exp[T]}. If the method accepts parameters having types \code{A1, ..., An} and has return type \code{R}, the corresponding lifted method will accept parameters having types \code{Exp[A1], ..., Exp[An]} and return type \code{Exp[R]}. However, \code{Exp[T]} also needs to support all methods that \code{T} inherits from its super-type \code{S}. To ensure this, we declare the type constructor \code{Exp} to be \emph{covariant} in its type parameter, so that \code{Exp[T]} correctly inherits the liftings from \code{Exp[S]}. This works even with the enrich-my-library pattern because implicit resolution respects subtyping in an appropriate way.

\smartParagraph{Limitations of Lifting}
Lifting methods of \code{Any} or \code{AnyRef} (Scala types at the root of the inheritance hierarchy) is not possible with this technique: \code{Exp[T]} inherits such methods and makes them directly available, hence the compiler will not insert an implicit conversion. Therefore, it is not possible to lift expressions such as \code{x == y}; rather, we have to rely on developer discipline to use \code{==\#} and \code{!=\#} instead of \code{==} and \code{!=}.

An expression like \code{"foo" + "bar" + str1} is converted to \code{toStringOps("foo" + "bar") + str1}; hence, part of the expression is evaluated before being reified. This is harmless here since we want \code{"foo" + "bar"} to be evaluated at compile-time, that is constant-folded, but in other cases it is preferable to prevent the constant folding. We will see later examples where queries on collections are evaluated before reification, defeating the purpose of our framework, and how we work around those.

\subsection{Lifting higher-order expressions}
\label{sec:lifting-ho}
We have shown how to lift first-order expressions; however, the interface of collections also uses higher-order methods, that is, methods that accept functions as parameters, and we need to lift them as well to reify the complete collection DSEL. For instance, the \code{map} method applies a function to each element of a collection. In this subsection, we describe how we reify such expressions of function type.

\smartParagraph{Higher-order abstract syntax}
To represent functions, we have to represent the bound variables in the function bodies. For example, a reification of \code{str => str + "!"} needs to reify the variable \code{str} of type \code{String} in the body of the anonymous function. This reification should retain the information where \code{str} is bound. We achieve this by representing bound variables using \emph{higher-order abstract syntax} (HOAS)~\citep{Pfenning88hoas}, that is, we represent them by variables bound at the meta level. To continue the example, the above function is reified as \code{(str: Exp[String]) => str + "!"}. Note how the type of \code{str} in the body of this version is \code{Exp[String]}, because \code{str} is a reified variable now. Correspondingly, the expression \code{str + "!"} is lifted as described in the previous subsection. 

With all operations in the function body automatically lifted, the only remaining syntactic difference between normal and lifted functions is the type annotation for the function's parameter. Fortunately, Scala's \emph{local type inference} can usually deduce the argument type from the context, for example, from the signature of the \code{map} operation being called. Type inference plays a dual role here: First, it allows the query writer to leave out the annotation, and second, it triggers lifting in the function body by requesting a lifted function instead of a normal function. This is how in Fig.~\ref{fig:reifiedQuery}, a single call to \code{asSquopt} triggers lifting of the overall query.

Note that reified functions have type \code{Exp[A] => Exp[B]} instead of the more regular \code{Exp[A => B]}. We chose the former over the latter to support Scala's syntax for anonymous functions and for-comprehensions which is hard-coded to produce or consume instances of the pre-defined \code{A => B} type. We have to reflect this irregularity in the lifting of methods and functions by treating the types of higher-order arguments accordingly.

\smartParagraph{User-defined methods, revised}
We can now extend the lifting of signatures for methods or functions from the previous subsection to the general case, that is, the case of higher-order functions. We lift a method or function with signature
\begin{lstlisting}
def m[A1, $...$, An](a1: T1, $...$, an: Tn): R
\end{lstlisting}
to a method or function with the following signature.
\begin{lstlisting}
def m[A1, $...$, An](a1: $\ExpWrap\llbracket$T1$\rrbracket$, $...$, an: $\ExpWrap\llbracket$Tn$\rrbracket$): $\ExpWrap\llbracket$R$\rrbracket$
\end{lstlisting}
As before, the definition of the lifted method or function will return an expression node representing the call. If the original was a function, the lifted version is also defined as a function. If the original was a method on type \code{T}, then the lifted version is enriched onto \code{T}.

The type transformation $\ExpWrap$ converts the argument and return types of the method or function to be lifted. For most types, $\ExpWrap$ just wraps the type in the \code{Exp} type constructor, but function types are treated specially: $\ExpWrap$ recursively descends into function types to convert their arguments separately. Overall, $\ExpWrap$ behaves as follows.

\begin{lstlisting}
$\ExpWrap\llbracket$(A1, ... , An) => R]$\rrbracket$ =
  ($\ExpWrap\llbracket$A1$\rrbracket$, $...$ , $\ExpWrap\llbracket$An$\rrbracket$ => $\ExpWrap\llbracket$R$\rrbracket$
$\ExpWrap\llbracket$A$\rrbracket$ = Exp[A]
\end{lstlisting}

We can use this extended definition of method lifting to  implement \code{map} lifting for \code{Lists}, that is, a method with signature \code{Exp[List[T]].map(Exp[T] => Exp[U])}:

\begin{lstlisting}
implicit def expToListOps[T](coll: Exp[List[T]]) = 
  new ListOps(coll)
implicit def toListOps[T](coll: List[T]) = 
  expToListOps(coll)
class ListOps(coll: Exp[List[T]]) {
  def map[U](f: Exp[T] => Exp[U]) =
    ListMapNode(coll, Fun(f))
}
case class ListMapNode[T, U](coll: Exp[List[T]], mapping: Exp[T => U]) extends Exp[List[U]]
\end{lstlisting}

Note how \code{map}'s parameter \code{f} has type \code{Exp[T] => Exp[U]} as necessary to enable Scala's syntax for anonymous functions and automatic lifting of the function body. This implementation would work for queries on lists, but does not support other collection types or queries where the collection type changes. We show in Sec.~\ref{subsec:collections} how {\LoS} integrates with such advanced features of the Scala Collection DSEL.

%
%
%
%
%
%
%
%
%

\subsection{Lifting collections}
\label{subsec:collections}
In this subsection, we first explain how for-comprehensions are desugared to calls to library functions, allowing an external library to give them a different meaning. We summarize afterwards needed information about the subset of the Scala collection DSEL that we reify. Then we present how we perform this reification.
We finally present the reification of the running example (Fig.~\ref{fig:reifiedQuery}).

%

%

\smartParagraph{For-comprehensions}
As we have seen, an idiomatic encoding in Scala of queries on collections are for-comprehensions. Although Scala is an impure functional language and supports side-effectful for-comprehensions, only pure queries are supported in our framework, because this enables or simplifies many domain-specific analyses. Hence we will restrict our attention to pure queries.

The Scala compiler desugars for-comprehensions into calls to three collection methods, \code{map}, \code{flatMap} and \code{withFilter}, which we explain shortly; the query in Fig.~\ref{fig:query} is desugared to the code in Fig.~\ref{fig:desugaredQuery}.
\begin{figure}
\begin{center}
\begin{lstlisting}
val records = books.
  withFilter(book => book.publisher == "Pearson Education").
  flatMap(book => book.authors.
  map(author => BookData(book.title,
    author.firstName + " " + author.lastName,
    book.authors.size - 1)))
\end{lstlisting}
\end{center}
\caption{Desugaring of code in Fig.~\ref{fig:query}.}
\label{fig:desugaredQuery}
\end{figure}

The compiler performs type inference and type checking on a for-comprehension only \emph{after} desugaring it; this affords some freedom for the types of \code{map}, \code{flatMap} and \code{withFilter} methods.

\smartParagraph{The Scala Collection DSEL}
A Scala collection containing elements of type \code{T} implements the trait \code{Traversable[T]}.
%
On an expression \code{coll} of type \code{Traversable[T]} one can invoke methods declared (in first approximation) as follows:
\begin{lstlisting}
def map[U](f: T => U): Traversable[U]
def flatMap[U](f: T => Traversable[U]): Traversable[U]
def withFilter[U](p: T => Boolean): Traversable[T].
\end{lstlisting}

For a Scala collection \code{coll}, the expression \code{coll.map(f)} applies \code{f} to each element of \code{coll}, collects the results in a new collection and returns it; \code{coll.flatMap(f)} applies \code{f} to each element of \code{coll}, concatenates the results in a new collection and returns it; \code{coll.withFilter(p)} produces a collection containing the elements of \code{coll} which satisfy the predicate \code{p}.

However, Scala supports many different collection types, and this complicates the actual types of these methods. Each collection can further implement subtraits like \code{Seq[T] <: Traversable[T]} (for sequences), \code{Set[T] <: Traversable[T]} (for sets) and \code{Map[K, V] <: Traversable[(K, V)]} (for dictionaries); for each such trait, different implementations are provided.

One consequence of this syntactic desugaring is that a single for-comprehension can operate over different collection types%
%
. The type of the result depends essentially on the type of the root collection, that is \code{books} in the example above. The example above can hence be altered to produce a sequence rather than a set by simply converting the root collection to another type:
\begin{lstlisting}
val recordsSeq = for {
   book <- books£\textbf{.toSeq}£
   if book.publisher == "Pearson Education"
   author <- book.authors
  } yield BookData(book.title,
    author.firstName + " " + author.lastName,
    book.authors.size - 1)
\end{lstlisting}

\smartParagraph{Precise static typing}
The Scala collections DSEL achieves precise static typing while avoiding code duplication~\citep{odersky2009fighting}. Precise static typing is necessary because the return type of a query operation can depend on subtle details of the base collection and query arguments. 
To return the most specific static type, the Scala collection DSL defines a type-level relation between the source collection type, the element type for the transformed collection, and the type for the resulting collection. The relation is encoded through the concept pattern~\citep{Oliveira10TCOI}, i.e., through a type-class-style trait \code{CanBuildFrom[From, Elem, To]}, and elements of the relation are expressed as implicit instances.

For example, a finite map can be treated as a set of pairs so that mapping a function from pairs to pairs over it produces another finite map. This behavior is encoded in an instance of type \code{CanBuildFrom[Map[K, V], (K1, V1), Map[K1, V1]}. The \code{Map[K, V]} is the type of the base collection, \code{(K1, V1)} is the return type of the function, and \code{Map[K1, V1]} is the return type of the map operation.

It is also possible to map some other function over the finite map, but the result will be a general collection instead of a finite map. This behavior is described by an instance of type \code{CanBuildFrom[Traversable[T], U, Traversable[U]}. Note that this instance is also applicable to finite maps, because \code{Map} is a subclass of \code{Traversable}. Together, these two instances describe how to compute the return type of mapping over a finite map.

\smartParagraph{Code reuse}
Even though these two use cases for mapping over a finite map have different return types, they are implemented as a single method that uses its implicit \code{CanBuildFrom} parameter to compute both the static type and the dynamic representation of its result. So the Scala Collections DSEL provides precise typing without code duplication. In our deep embedding, we want to preserve this property.

\code{CanBuildFrom} is used in the implementation of \code{map}, \code{flatMap} and \code{withFilter}. To further increase reuse, the implementations are provided in a helper trait \code{TraversableLike[T, Repr]}, with the following signatures:

\begin{lstlisting}
def map[U](f: T => U)
  (implicit cbf: CanBuildFrom[Repr, U, That]): That
def flatMap[U](f: T => Traversable[U])
  (implicit cbf: CanBuildFrom[Repr, U, That]): That
def withFilter[U](p: T => Boolean): Repr.
\end{lstlisting}

The \code{Repr} type parameter represents the specific type of the receiver of the method call.

\smartParagraph{The lifting}
The basic idea is to use the enrich-my-library pattern to lift collection methods from \code{TraversableLike[T, Repr]} to \code{TraversableLikeOps[T, Repr]}:
\begin{lstlisting}
implicit def expToTraversableLikeOps[T, Repr]
  (v: Exp[TraversableLike[T, Repr]]) =
  new TraversableLikeOps[T, Repr](v)
\end{lstlisting}

However, given the design of the collection library, every instance of \code{TraversableLike[T, Repr]} is also an instance of both \code{Traversable[T]} and \code{Repr}; to take advantage of this during interpretation and optimization, we need to restrict the type of \code{expToTraversableLikeOps}, getting the following conversion:\footnote{Due to type inference bugs, the actual implicit conversion needs to be slightly more complex, to mention \code{T} directly in the argument type. We reported the bug at \url{https://issues.scala-lang.org/browse/SI-5298}.}

%
%
%
\begin{lstlisting}
implicit def expToTraversableLikeOps
  [T, Repr <: Traversable[T]
                with TraversableLike[T, Repr]]
  (v: Exp[Repr]) =
    new TraversableLikeOps[T, Repr](v)
\end{lstlisting}

The query operations are defined in class \code{TraversableLikeOps[T, Repr]}; a few examples are shown in Fig.~\ref{fig:liftTrav}.%
\footnote{Similar liftings are introduced for traits similar to \code{TraversableLike}, like \code{SeqLike}, \code{SetLike}, \code{MapLike}, and so on.}

Note how the lifted query operations use \code{CanBuildFrom} to compute the same static return type as the corresponding non-lifted query operation would compute. This reuse of type-level machinery allows {\LoS} to provide the same interface as the Scala Collections DSEL.

\smartParagraph{Code reuse, revisited}
We already saw how we could reify \code{List[T].map} through a specific expression node, \code{ListMapNode}. However, this approach would require generating many variants for different collections with slightly different types; writing an optimizer able to handle all such variations would be unfeasible because of the amount of code duplication required.
Instead, by reusing Scala type-level machinery, we obtain a reification which is statically typed and at the same time avoids code duplication in both our lifting and our optimizer, and in general in all possible consumers of our reification, making them feasible to write.

%
%
%

%
%

\begin{figure}
\begin{center}
\begin{lstlisting}
class TraversableLikeOps[T, Repr <: Traversable[T]
        with TraversableLike[T, Repr]](t: Exp[Repr]) {
  val t: Exp[Repr]
  def withFilter(f: Exp[T] => Exp[Boolean]): Exp[Repr] =
    Filter(this.t, FuncExp(f))
  def map[U, That <: TraversableLike[U, That]]
         (f: Exp[T] => Exp[U])
         (implicit c: CanBuildFrom[Repr, U, That]):
         Exp[That] =
    MapNode(this.t, FuncExp(f))
  //... other methods ...
}
//definitions of MapNode, Filter omitted.
\end{lstlisting}
\end{center}
\caption{Lifting \code{TraversableLike}}
\label{fig:liftTrav}
\end{figure}

%
\pg{Discuss asSquopt if possible! Start from the commented out paragraph I added; otherwise, remove the dangling pointer to here from before.}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%

%

%
%
%

%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\subsection{Interpretation}
\label{sec:interpretation}

After optimization, {\LoS} needs to interpret the optimized expression trees to perform the query. Therefore, the trait \code{Exp[T]} declares an \code{def interpret(): T} method, and each expression node overrides it appropriately to implement a mostly standard typed, tagless~\citep{carette09finally}, environment-based interpreter. The interpreter computes a value of type \code{T} from an expression tree of type \code{Exp[T]}. This design allows query writers to extend the interpreter to handle application-specific operations. In fact, the lifting generator described in Sec.~\ref{sec:lifting-ho} automatically generates appropriate definitions of \code{interpret} for the lifted operations. 

For example, the interpretation of string concatenation is simply string concatenation, as shown in the following fragment of the interpreter. Note that type-safety of the interpreter is checked automatically by the Scala compiler when it compiles the fragments.

\begin{lstlisting}
case class StringConcat(str1: Exp[String],
    str2: Exp[String]) extends Exp[String] {
  def interpret() = str1.interpret() + str2.interpret()
}
\end{lstlisting}

The subset of Scala we reify roughly corresponds to a typed lambda calculus with subtyping and type constructors. It does not include constructs for looping or recursion, so it should be strongly normalizing as long as application programmers do not add expression nodes with non-terminating interpretations. However, query writers can use the host language to create a reified expression of infinite size. This should not be an issue if {\LoS} is used as a drop-in replacement for the Scala Collection DSEL.

During optimization, nodes of the expression tree might get duplicated, and the
interpreter could, in principle, observe this sharing and treat the expression
tree as a DAG, to avoid recomputing results. Currently, we do not exploit this,
unlike during compilation.

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

\subsection{Optimization}
%
%
%
%
%

\label{subsec:transf}
%

%
Our optimizer is structured as a pipeline of different transformations on a single intermediate representation, constituted by our expression trees.
Each phase of the pipeline, and the pipeline as a whole, produce a new expression having the same type as the original one.
Most of our transformations express simple rewrite rules with or without side conditions, which are applied on expression trees from the bottom up and are implemented using Scala's support for pattern matching~\citep{Emir07Patterns}.

%
%
%

%
%

%
Some optimizations, like filter hoisting (which we applied manually to produce the code in Fig.~\ref{fig:titleFilterho2}),
are essentially domain-specific and can improve complexity of a query. To enable such optimizations to trigger, however, one needs often to perform inlining-like transformations and to simplify the result. Inlining-related transformation can for instance produce code like \code{(x, y)._1}, which we simplify to \code{x}, reducing abstraction overhead but also (more importantly) making syntactically clear that the result does not depend on \code{y}, hence might be computed before \code{y} is even bound. This simplification extends to user-defined product types; with definitions in Fig.~\ref{fig:schema} code like \code{BookData(book.title, ...).title} is simplified to \code{book.title}.
%

We have implemented thus optimizations of three classes:
\begin{itemize}
\item general-purpose simplifications, like inlining, compile-time beta-reduction, constant folding and reassociation on primitive types, and other simplifications\footnote{Beta-reduction and simplification are run in a fixpoint loop~\citep{Peyton-Jones02}. Termination is guaranteed because our language does not admit general recursion.}; 
\item domain-specific simplifications, whose main goal is still to enable more important optimizations;
\item domain-specific optimizations which can change the complexity class of a query, such as filter hoisting, hash-join transformation or indexing.
\end{itemize}

\pg{Clarify the following paragraph. Just explain the optimizations properly in the ICSE submission.}
Among domain-specific simplifications, we implement a few described in the context of the monoid comprehension calculus~\citep{Grust96Translating,Grust99PhD}, such as query unnesting and fusion of bulk operators. Query unnesting allows to \emph{unnest} a for comprehension nested inside another, and produce a single for-comprehension.
Furthermore, we can fuse different collection operations together: collection operators like \code{map}, \code{flatMap} and \code{withFilter} can be expressed as folds producing new collections which can be combined.
Scala for-comprehension are however more general than monoid comprehensions\footnote{For instance, a for-comprehension producing a list cannot iterate over a set.}, hence to ensure safety of some optimizations we need some additional side conditions\footnote{For instance, consider a for-comprehension producing a set and nested inside another producing a list. This comprehension does not correspond to a valid monoid comprehension (see previous footnote), and query unnesting does not apply here: if we unnested the inner comprehension into the outer one, we would not perform duplicate elimination on the inner comprehension, affecting the overall result.}.

%
\smartParagraph{Manipulating functions}
%
%
To be able to inspect a HOAS function body \code{funBody: Exp[S] => Exp[T]}, like \code{str => str + "!"}, we convert it to \emph{first-order} abstract syntax (FOAS), that is to an expression tree of type \code{Exp[T]}.
To this end, we introduce a representation of variables and a generator of fresh ones; since variable names are auto-generated, they are internally represented simply as integers instead of strings for efficiency.

To convert \code{funBody} from HOAS to FOAS we apply it to a fresh variable \code{v} of type \code{TypedVar[S]}, obtaining a first-order representation of the function body, having type \code{Exp[T]}, and containing occurrences of \code{v}.

This transformation is hidden into the constructor \code{Fun}, which converts \code{Exp[S] => Exp[T]}, a representation of an expression with one free variable, to \code{Exp[S => T]}, a representation of a function.

\begin{lstlisting}
case class App[S, T](f: Exp[S => T], t: Exp[S]) extends Exp[T]
def Fun[-S, +T](f: Exp[S] => Exp[T]): Exp[S => T] = {
  val v = Fun.gensym[S]()
  FOASFun(funBody(v), v)
}
case class FOASFun[S, T](val foasBody: Exp[T], v: TypedVar[S]) extends Exp[S => T]
implicit def app[S, T](f: Exp[S => T]): Exp[S] => Exp[T] =
  arg => App(f, arg)
\end{lstlisting}

Conversely, function applications are represented using the constructor \code{App}; an implicit conversion allows \code{App} to be inserted implicitly. Whenever \code{f} can be applied to \code{arg} and \code{f} is an expression tree, the compiler will convert \code{f(arg)} to \code{app(f)(arg)}, that is \code{App(f, arg)}.

%

%
%
%
In our example, \code{Fun(str => str + "!")} produces \code{FOASFun(StringConcat(TypedVar[String](1), Const("!")), TypedVar[String](1))}%
%
.

\pg{Comment back in the following discussion, if it can be made good.}
%
%
%
%
%
%

Since we auto-generate variable names, it is easiest to implement represent variable occurrences using the Barendregt convention, where bound variables must always be globally unique; we must be careful to perform renaming after beta-reduction to restore this invariant~\citep[Ch.~6]{Pierce02TAPL}.

We can now easily implement substitution and beta-reduction and through that, as shown before, enable other optimizations to trigger more easily and speedup queries.

%
%

%

%

%
%
%
%
%
%
%
%
%
%


%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%



%
%
%

%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

